A kinetic model for polyatomic gas with quasi-resonant collisions leading to bi-temperature relaxation processes

In this article, we extend the Boltzmann framework for polyatomic gases by introducing quasi-resonant kernels, which relax resonant interactions, for which kinetic and internal energies are separately conserved and lead to equilibrium states with two temperatures. We establish an H-theorem and analyze the quasi-resonant model's asymptotic behaviour, demonstrating a two-phase relaxation process: an initial convergence towards a two-temperature Maxwellian state followed by gradual relaxation of the two temperatures towards each other. Numerical simulations validate our theoretical predictions. The notion of quasi-resonance provides the first rigorous framework of a Boltzmann dynamics for which the distribution is at all times close to a multi-temperature Maxwellian, relaxing towards a one-temperature Maxwellian.

==> collisionresonante.tex <==
\begin{tikzpicture}[scale=.4]
\tikzset{molecule/.pic={code= \tikzset{scale=.04}
    %Atomes
    \shade[ball color=red] (-4,0) circle (4);
    \shade[ball color=black!80] (0,0) circle (5);
    \shade[ball color=red] (4,0) circle (4);}}
    
    \path (0,2) pic[rotate=235]{molecule};
    \path (0,-2) pic[rotate=305]{molecule};
    \draw[draw=none, fill=white, opacity = .3] (-.8,-2.8) rectangle (1,2.8);
    
    \draw[->,thick] (1,1.3)--(2.5,.4);
    \draw[->,thick] (1,-1.3)--(2.5,-.4);
    \path (4.8,2.5) pic[rotate=315]{molecule};
    \path (4.8,-2.5) pic[rotate=225]{molecule};
    \draw[->,thick] (3.5,.4) -- (4.5,2);
    \draw[->,thick] (3.5,-.4) -- (4.5,-2);    
    \draw (3,0) node{$\star$};   
    \draw (1.6,2) node{$v,I$};


    \draw (2,-2) node{$v_*,I_*$};
    \draw (5.4,1.3) node{$v',I'$};
    \draw (5.4,-1.3) node{$v'_*,I'_*$}; 
\end{tikzpicture}
